Grounded Adjudication of Variations across Extracted TimeLines (GAVEL): Comparing Clinical Timelines Against Their Case Reports

Existing pipelines for clinical timeline extraction from case reports are evaluated using an expert reference and are limited by imperfect reference annotations and imprecise event alignment. We developed GAVEL, an LLM judge protocol that compares two timelines with the case report and returns a discrepancy type, verdict, and report passage for each difference. We evaluated the event matcher, reviewed 2,738 findings from GPT5.6sol and DeepSeek V3.2, ranked six LLM extractors and two human annotators, and tested GAVEL guided merging. True match rates were 60% immediately below and 48% immediately above the 0.10 cutoff. Manual review confirmed 89.4% and 88.6% of findings. Across 126 reports, merged timelines were preferred in 77.0% of comparisons (95% CI, 69.8 to 84.1%) and reduced discrepancies attributed to the evaluated timeline from 7.63 to 0.85 per report. GAVEL supports report-based comparison and revision without treating either timeline as ground truth.

==> discussion_old.tex <==
\section*{Discussion} 

GAVEL addresses a measurement problem in clinical timeline extraction: existing evaluations require both an event-alignment rule and a privileged reference timeline before correctness can be assessed. Our results show that uncertainty enters at both points. PubMedBERT cosine distance separated clear matches from clear mismatches at the extremes, but true and false alignments remained substantially interleaved around the operational threshold. Source-grounded pairwise adjudication provided a different form of evidence. Among findings emitted by GAVEL, 89.4\% from GPT-5.6-sol and 88.6\% from DeepSeek V3.2 were confirmed by manual review, and the resulting findings supported comparisons among six LLM extractors and two human annotators without designating any candidate timeline as gold. The same findings could also be converted into proposed corrections: merged timelines were preferred to the leading single-source timeline in 77.0\% of reports and received substantially fewer charged discrepancies. 

The matcher audit demonstrates why improving only the final summary metric is insufficient. An event-recovery or temporal-agreement score is conditioned on the alignments supplied to it; when the matcher confuses corresponding and noncorresponding events near its decision boundary, downstream scores inherit that uncertainty. Changing the threshold may alter the balance between retained false matches and discarded true matches, but it does not determine which event, value, or timestamp is supported by the source. GAVEL shifts that decision from embedding proximity to documentary evidence and exposes the basis for each verdict. It does not eliminate every measurement choice---the discrepancy schema, temporal tolerance, and scoring rule remain prespecified design decisions---but it makes those choices explicit and keeps the source evidence attached to the resulting judgment. 

GAVEL also occupies a different position from existing LLM-based evaluators. General-purpose pairwise judges estimate which response is preferable and can be influenced by position, style, verbosity, and model-family effects \cite{zheng2023judging,chiang2024chatbotarena,panickssery2024selfpreference}. Source-grounded factuality methods instead determine whether claims in one generated document are supported by an external knowledge source or a patient's record \cite{min2023factscore,chung2025verifying}. TIMER evaluates temporal reasoning over longitudinal clinical records, but its unit of analysis is a free-text answer rather than a disagreement between two structured timelines \cite{cui2025timer}. GAVEL combines these previously separate elements: pairwise comparison, patient-specific source grounding, explicit event-time reasoning, and typed adjudication at the level of individual discrepancies. The criterion is not which timeline is more fluent or comprehensive, but which account of a disputed event the available report evidence supports. 

Placing both human annotators on the same leaderboard illustrates the practical consequence of removing the privileged reference. The 201-point separation between A1 and A2 does not establish that one annotator is generally more clinically capable, nor does the placement of several models above an annotator establish broad model superiority. It shows that, on this corpus and under the published temporal conventions, the choice of human reference materially changes the standard against which every extractor is evaluated. Reference-based evaluation absorbs this variation into model scores; GAVEL measures it directly. The corpus-scale comparison further showed that similar aggregate ratings can conceal different failure modes. GLM-5.2 placed events more accurately in time but omitted more supported events, whereas A1 recovered more events but incurred more timing and duplicate findings. GPT-5 led because it balanced event recovery and temporal placement rather than dominating every error category.

These error profiles are more actionable than a single ranking. In both evaluation stages, omissions and timing errors were substantially more common than unsupported additions. For this corpus, improving event recall and temporal anchoring may therefore yield greater benefit than focusing exclusively on hallucination suppression. The findings also qualify how nondecisive judgments should be interpreted. Nearly one-third of Stage 3 findings did not favor either candidate under the scoring rule, but this group includes clinically equivalent representations, content unsupported in both timelines, and genuinely unresolved cases. It should not be interpreted uniformly as source ambiguity. Instead, the availability of \texttt{BOTH}, \texttt{NEITHER}, and \texttt{UNCLEAR} allows the evaluator to avoid forcing a winner when the evidence does not justify one. 

The two judge families produced similar confirmation rates but different numbers and types of findings. DeepSeek V3.2 emitted 342 fewer findings than GPT-5.6-sol, and the principal residual errors differed across models: GPT-5.6-sol more often undercalled unsupported additions, whereas DeepSeek V3.2 more often missed one-sided discrepancies. Similar conditional confirmation rates therefore suggest that the protocol can be applied across model families, but they do not establish equal discrepancy coverage or prove that the protocol itself is correct. The leading shared failure was overuse of \texttt{UNCLEAR} for timing disagreements that the reviewer considered resolvable. This concentration is useful because it identifies a specific behavior for further prompt or rule refinement, but such refinement must be evaluated on held-out cases rather than on the examples that motivated it. \textcolor{blue}{In the blinded second-reviewer analysis, [insert confirmation rate, agreement between reviewers, and whether the same dominant error categories were reproduced].} 

The merge experiment indicates that typed adjudications can serve as more than an evaluation report. Folding supported information from a complementary timeline into the leading timeline reduced the judge-charged discrepancy rate from 7.63 to 0.85 per report, with the largest reductions in missed events and incorrect times. The small increases in false duplicates and missed recurrences show that merging was not uniformly beneficial, but the overall pattern is consistent with the complementary error profiles identified in the leaderboard. This result supports a workflow in which multiple extractors generate candidate timelines, GAVEL localizes their disagreements, and a merger incorporates only source-supported information. Nevertheless, the merge result measures preference under a second LLM judge, not independent clinical correctness. Separating generation and final adjudication across GPT and DeepSeek families reduces direct self-evaluation but cannot eliminate correlated model errors. \textcolor{blue}{Manual review of the eight pilot merges found [insert edit-application fidelity and number of timelines with silently dropped or altered unaffected events].} 

The broader implication is that timeline evaluation should distinguish documentary fidelity from agreement with one annotation. Extracted timelines may subsequently support phenotyping, trajectory modeling, and time-to-event analyses \cite{estiri2021temporal,kumar2026glp1ra}; errors in event inclusion or temporal placement can therefore propagate into downstream estimates. GAVEL provides an auditable quality-control layer that identifies the disputed event, records the direction of error, and links the verdict to the underlying evidence. The present study does not establish that GAVEL-corrected timelines improve a downstream clinical model. Evaluating changes in time-to-event estimates, risk models, or phenotype assignments is an important next step. 

\vspace{-2.5mm}
\paragraph{Limitations and Future Directions} 

This study has several limitations. First, the evaluation corpus comprises published GLP-1RA case reports, which are relatively self-contained narratives written for human readers. Performance may differ on fragmented EHR notes, longitudinal records spanning many encounters, or documents containing contradictory entries. The report is also an evidentiary source rather than infallible clinical ground truth: an event omitted from or incorrectly described in the publication cannot be recovered through source grounding. GAVEL evaluates support within the available document and should not be interpreted as reconstructing unobserved clinical truth. Second, the matcher audit used a balanced sample of 100 pairs, with only 25 pairs per distance band. Its confidence intervals are consequently wide, and because sampling was stratified rather than prevalence-weighted, the observed band proportions do not estimate the corpus-wide alignment error rate. A larger independently labeled sample would support calibration analysis and direct comparison with stronger cross-encoder or LLM-based event matchers. Third, manual validation began with findings emitted by the judge. The reported confirmation rates therefore measure correctness among reported discrepancies but do not measure recall for discrepancies that GAVEL failed to identify. Most findings were assessed by one primary reviewer who could see the judge verdict and supporting evidence, which may influence borderline decisions; the blinded second-reviewer study addresses this concern only on a stratified subset. Automated confirmation that an evidence string occurs in the report verifies extractive grounding, not that the quoted sentence entails the verdict. A stronger validation would require independent reviewers to construct a complete discrepancy set on held-out reports, permitting separate estimates of detection precision, recall, discrepancy-type accuracy, verdict accuracy, and evidence validity. Fourth, leaderboard results depend on the cases, opponents, judge, timing tolerance, and scoring conventions used. The full eight-source round robin contained only 15 independent reports, although the corpus-scale analysis provided greater precision for three selected entrants. Charged findings are pairwise discrepancy instances rather than deduplicated unique timeline errors, so one underlying error can be observed against multiple opponents. Non-preference-bearing findings were excluded from ratings, and alternative treatments of \texttt{UNCLEAR}, discrepancy weights, or temporal tolerance could affect close comparisons. Position-swapped evaluations, additional judge families, and sensitivity analyses over these choices would provide stronger evidence of ranking stability. Finally, pairwise adjudication can identify only differences visible between the candidate timelines. An event omitted by both candidates, or the same incorrect value or time reproduced by both, may pass through without a finding and cannot be repaired by the merge. Future work should combine GAVEL with independent source-event coverage audits, extend it to discharge summaries and longitudinal EHRs, evaluate human review targeted to unresolved findings, and measure whether adjudicated timelines improve downstream temporal analyses.

==> table12_combined.tex <==
\begin{table}[H]
\centering

% =========================
% LEFT: Judge validation
% =========================
\begin{minipage}[t]{0.40\linewidth}
\vspace{0pt}
\captionsetup{font=footnotesize,labelfont=bf,skip=2pt}
\captionof{table}{Manual review of emitted GAVEL findings by judge family.}
\label{tab:judge_validation}
\centering
\renewcommand{\arraystretch}{0.94}
\setlength{\tabcolsep}{2.2pt}

\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lrrr@{}}
\toprule
\textbf{Error type}
& \textbf{GPT-5.6-sol}
& \textbf{DeepSeek V3.2}
& \textbf{Total} \\
\midrule
Timing ruled unclear
& 59 & 67 & 126 \\
Undercalled over-extraction
& 64 & 9 & 73 \\
Anchor forced on two-sided case
& 21 & 14 & 35 \\
Missed one-sided finding
& 1 & 13 & 14 \\
Overcalled duplicate
& 7 & 7 & 14 \\
Perception timing
& 6 & 8 & 14 \\
Other (5 categories)
& 2 & 13 & 15 \\
Value miscalled
& 4 & 6 & 10 \\
\midrule
\textbf{Total errors}
& \textbf{164}
& \textbf{137}
& \textbf{301} \\
\textbf{Findings reviewed}
& \textbf{1,540}
& \textbf{1,198}
& \textbf{2,738} \\
\textbf{Confirmation rate}
& \textbf{89.4\%}
& \textbf{88.6\%}
& \textbf{89.0\%} \\
\bottomrule
\end{tabular}%
}
\end{minipage}
\hfill
% =========================
% RIGHT: Stage 2 + Stage 3
% =========================
\begin{minipage}[t]{0.56\linewidth}
\vspace{0pt}
\captionsetup{font=footnotesize,labelfont=bf,skip=2pt}
\captionof{table}{Charged pairwise discrepancy instances by entrant. Stage 2 rates are per report across seven opponents; Stage 3 rates are per entrant--report matchup.}
\label{tab:error_profiles}
\centering
\renewcommand{\arraystretch}{0.91}
\setlength{\tabcolsep}{1.3pt}

\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
\textbf{Entrant}
& \shortstack{\textbf{Wrong}\\\textbf{time}}
& \shortstack{\textbf{Missed}\\\textbf{positive}}
& \shortstack{\textbf{Missed}\\\textbf{negative}}
& \shortstack{\textbf{Missed}\\\textbf{recurrence}}
& \shortstack{\textbf{Wrong}\\\textbf{value}}
& \shortstack{\textbf{False}\\\textbf{duplicate}}
& \shortstack{\textbf{Over-}\\\textbf{annotated}}
& \textbf{Total} \\
\midrule

\multicolumn{9}{@{}l}{\textit{A. Eight-source round robin}} \\
GPT-5
& 2.6 & 2.7 & 0.2 & 0.0 & 0.0 & 0.3 & 0.2 & 6.0 \\
Claude Opus 5
& 1.4 & 5.1 & 0.2 & 0.1 & 0.1 & 0.3 & 0.0 & 7.2 \\
o4-mini
& 0.9 & 5.0 & 0.7 & 0.0 & 0.1 & 0.3 & 0.1 & 7.1 \\
Annotator 1 (A1)
& 3.3 & 2.6 & 0.6 & 0.0 & 0.5 & 0.3 & 0.1 & 7.4 \\
GLM-5.2
& 3.2 & 5.7 & 0.4 & 0.1 & 0.7 & 0.7 & 0.1 & 10.9 \\
Gemma 4
& 4.1 & 7.5 & 1.2 & 0.1 & 0.9 & 0.1 & 0.1 & 14.0 \\
Annotator 2 (A2)
& 5.2 & 8.1 & 0.6 & 0.0 & 1.5 & 0.5 & 0.1 & 16.0 \\
Llama 3.3 70B
& 17.4 & 11.7 & 3.1 & 0.7 & 1.3 & 0.3 & 0.1 & 34.6 \\
\cmidrule(lr){1-9}
\emph{Mean entrant}
& \emph{4.8}
& \emph{6.1}
& \emph{0.9}
& \emph{0.1}
& \emph{0.6}
& \emph{0.3}
& \emph{0.1}
& \emph{12.9} \\

\addlinespace[3pt]
\multicolumn{9}{@{}l}{\textit{B. Corpus-scale comparison}} \\
GPT-5
& 3.7 & 3.2 & 0.4 & 0.1 & 0.1 & 0.5 & 0.2 & 8.1 \\
GLM-5.2
& 2.6 & 11.5 & 1.4 & 0.3 & 0.5 & 0.3 & 0.0 & 16.7 \\
Annotator 1 (A1)
& 5.5 & 5.5 & 1.2 & 0.1 & 0.8 & 1.1 & 0.3 & 14.6 \\
\cmidrule(lr){1-9}
\emph{Mean entrant}
& \emph{3.9}
& \emph{6.8}
& \emph{1.0}
& \emph{0.1}
& \emph{0.5}
& \emph{0.6}
& \emph{0.2}
& \emph{13.1} \\

\bottomrule
\end{tabular}%
}
\end{minipage}

\end{table}
